Efficient mesh management in Firedrake using PETSc-DMPlex

The use of composable abstractions allows the application of new and established algorithms to a wide range of problems while automatically inheriting the benefits of well-known performance optimisations. This work highlights the composition of the PETSc DMPlex domain topology abstraction with the Firedrake automated finite element system to create a PDE solving environment that combines expressiveness, flexibility and high performance. We describe how Firedrake utilises DMPlex to provide the indirection maps required for finite element assembly, while supporting various mesh input formats and runtime domain decomposition. In particular, we describe how DMPlex and its accompanying data structures allow the generic creation of user-defined discretisations, while utilising data layout optimisations that improve cache coherency and ensure overlapped communication during assembly computation.

==> figures/plex_graph_api.tex <==
\begin{figure}[ht]
  \centering
  \begin{subfigure}{0.3\textwidth}
    \centering
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_simple}
    \end{tikzpicture}
    \caption{\centering Entity numbering for a single tetrahedron}
    \label{fig:tet_simple}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \centering
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift=-3pt, yshift=-3pt] 1.south west) --
        ([xshift= 3pt, yshift=-3pt] 4.south east) --
        ([xshift= 3pt, yshift= 3pt] 4.north east) --
        ([xshift=-3pt, yshift= 3pt] 1.north west) --
        cycle;
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $stratum_{height}(1) = \{1, 2, 3, 4\}$}
    \label{fig:tet_height}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \centering
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift=-3pt, yshift=-3pt] 11.south west) --
        ([xshift= 3pt, yshift=-3pt] 14.south east) --
        ([xshift= 3pt, yshift= 3pt] 14.north east) --
        ([xshift=-3pt, yshift= 3pt] 11.north west) --
        cycle;
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $stratum_{depth}(0) = \{11, 12, 13, 14\}$}
    \label{fig:tet_depth}
  \end{subfigure}
  \vspace{6mm}

  \begin{subfigure}{0.3\textwidth}
    \centering
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift= 3pt, yshift=-3pt] 7.south east) --
        ([xshift= 3pt, yshift= 3pt] 7.north east) --
        ([xshift=-3pt, yshift= 3pt] 5.north west) --
        ([xshift=-3pt, yshift=-3pt] 5.south west) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (1.center) {};
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $cone(1) = \linebreak\{5, 6, 7\}$}
    \label{fig:tet_cone}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \hspace{7.3mm}
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift= 3pt, yshift=-3pt] 10.south east) --
        ([xshift= 3pt, yshift= 3pt] 10.north east) --
        ([xshift=-3pt, yshift= 3pt] 8.north west) --
        ([xshift=-3pt, yshift=-3pt] 8.south west) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (14.center) {};
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $support(14) = \linebreak\{8, 9, 10\}$}
    \label{fig:tet_support}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \hspace{7.3mm}
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift= 1pt, yshift=-3pt] 1.south east) --
        ([xshift=-3pt, yshift= 1pt] 2.north west) --
        ([xshift= 3pt, yshift=-1pt] 7.south east) --
        ([xshift=-3pt, yshift= 1pt] 8.north west) --
        ([xshift= 3pt, yshift=-1pt] 13.south east) --
        ([xshift= 3pt, yshift= 3pt] 13.north east) --
        ([xshift=-2pt, yshift= 3pt] 11.north west) --
        ([xshift=-2pt, yshift= 0pt] 5.west) --
        ([xshift=-1pt, yshift=-3pt] 1.south west) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (1.center) {};
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $closure(1) = \{1, 5, 6, 7, 11, 12, 13\}$}
    \label{fig:tet_closure}
  \end{subfigure}
  \vspace{6mm}

  \begin{subfigure}{0.3\textwidth}
    \hspace{7.3mm}
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift= 0pt, yshift= 3pt] 14.north west) --
        ([xshift= 3pt, yshift=-3pt] 13.south east) --
        ([xshift=-3pt, yshift= 1pt] 8.north west) --
        ([xshift= 3pt, yshift=-1pt] 7.south east) --
        ([xshift=-3pt, yshift= 1pt] 2.north west) --
        ([xshift=-3pt, yshift= 1pt] 2.south west) --
        ([xshift= 0pt, yshift=-3pt] 0.south west) --
        ([xshift= 0pt, yshift=-3pt] 0.south east) --
        ([xshift= 3pt, yshift=-1pt] 4.south east) --
        ([xshift= 3pt, yshift= 0pt] 10.east) --
        ([xshift= 2pt, yshift= 3pt] 14.north east) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (14.center) {};
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $star(14) = \{0, 2, 3, 4, 8, 9, 10, 14\}$}
    \label{fig:tet_star}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \hspace{7.3mm}
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift= 1pt, yshift=-3pt] 1.south east) --
        ([xshift=-3pt, yshift= 1pt] 2.north west) --
        ([xshift= 3pt, yshift=-1pt] 7.south east) --
        ([xshift=-3pt, yshift= 1pt] 8.north west) --
        ([xshift= 3pt, yshift=-1pt] 13.south east) --
        ([xshift= 2pt, yshift= 3pt] 13.north east) --
        ([xshift=-2pt, yshift= 3pt] 11.north west) --
        ([xshift=-2pt, yshift= 0pt] 5.west) --
        ([xshift=-1pt, yshift=-3pt] 1.south west) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (1.center) {};
      \end{scope}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift= 1pt, yshift=-3pt] 3.south east) --
        ([xshift=-3pt, yshift= 3pt] 4.north west) --
        ([xshift= 3pt, yshift=-1pt] 10.south east) --
        ([xshift= 2pt, yshift= 3pt] 14.north east) --
        ([xshift= 0pt, yshift= 3pt] 14.north west) --
        ([xshift=-3pt, yshift= 1pt] 9.north west) --
        ([xshift= 3pt, yshift=-3pt] 8.south east) --
        ([xshift=-3pt, yshift=-3pt] 8.south west) --
        ([xshift=-3pt, yshift= 1pt] 8.north west) --
        ([xshift= 2pt, yshift= 3pt] 12.north east) --
        ([xshift=-2pt, yshift= 3pt] 11.north west) --
        ([xshift=-3pt, yshift=-3pt] 11.south west) --
        ([xshift= 3pt, yshift= 1pt] 6.north east) --
        ([xshift=-3pt, yshift=-1pt] 7.south west) --
        ([xshift= 3pt, yshift= 3pt] 2.north east) --
        ([xshift=-1pt, yshift=-3pt] 3.south west) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (3.center) {};
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $meet(1, 3) = \linebreak\{7, 11, 12\}$}
    \label{fig:tet_meet}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \hspace{7.3mm}
    \begin{tikzpicture}[scale=1.2]
      \input{figures/tet_graph}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift=-1pt, yshift= 3pt] 11.north) --
        ([xshift=-3pt, yshift= 1pt] 11.west) --
        ([xshift= 2pt, yshift= 2pt] 5.east) --
        ([xshift=-2pt, yshift=-2pt] 1.west) --
        ([xshift= 0pt, yshift=-3pt] 0.south west) --
        ([xshift= 0pt, yshift=-3pt] 0.south east) --
        ([xshift= 3pt, yshift=-1pt] 3.south east) --
        ([xshift= 3pt, yshift= 2pt] 9.south east) --
        ([xshift= 3pt, yshift= 3pt] 9.north east) --
        ([xshift=-3pt, yshift= 3pt] 9.north west) --
        ([xshift= 3pt, yshift=-3pt] 8.south east) --
        ([xshift=-3pt, yshift=-3pt] 8.south west) --
        ([xshift=-3pt, yshift= 1pt] 8.north west) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (11.center) {};
      \end{scope}
      \begin{scope}[overlay, remember picture, rounded corners]
        \filldraw[fill opacity=0.2]
        ([xshift= 0pt, yshift= 3pt] 14.north west) --
        ([xshift= 3pt, yshift=-3pt] 13.south east) --
        ([xshift=-3pt, yshift= 1pt] 8.north west) --
        ([xshift= 3pt, yshift=-1pt] 7.south east) --
        ([xshift=-3pt, yshift= 1pt] 2.north west) --
        ([xshift=-3pt, yshift=-1pt] 2.south west) --
        ([xshift= 0pt, yshift=-3pt] 0.south west) --
        ([xshift= 0pt, yshift=-3pt] 0.south east) --
        ([xshift= 3pt, yshift=-1pt] 4.south east) --
        ([xshift= 3pt, yshift= 0pt] 10.east) --
        ([xshift= 2pt, yshift= 3pt] 14.north east) --
        cycle;
        \node[cell, fill=black, opacity=0.6] at (14.center) {};
      \end{scope}
    \end{tikzpicture}
    \caption{\centering $join(14, 11) = \linebreak\{0, 2, 3, 9\}$}
    \label{fig:tet_join}
  \end{subfigure}

\end{figure}

